ILC Reference Design Report Volume 3 - Accelerator

The International Linear Collider (ILC) is a 200-500 GeV center-of-mass high-luminosity linear electron-positron collider, based on 1.3 GHz superconducting radio-frequency (SCRF) accelerating cavities. The ILC has a total footprint of about 31 km and is designed for a peak luminosity of 2x10^34 cm^-2 s^-1. The complex includes a polarized electron source, an undulator-based positron source, two 6.7 km circumference damping rings, two-stage bunch compressors, two 11 km long main linacs and a 4.5 km long beam delivery system. This report is Volume III (Accelerator) of the four volume Reference Design Report, which describes the design and cost of the ILC.

==> EDR/resetcounters.tex <==
%\setcounter{page}{1}
%\setcounter{figure}{0}
%\setcounter{table}{0}
\setcounter{secnumdepth}{4}
\setcounter{subsection}{0} 
\setcounter{subsubsection}{0}
\usecounter{subsubsection}

==> Overview/resetcounters.tex <==
%\setcounter{page}{1}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{secnumdepth}{4}
\setcounter{subsection}{0} 
\setcounter{subsubsection}{0}
\usecounter{subsubsection}

==> cfs/resetcounters.tex <==
%\setcounter{page}{1}
%\setcounter{figure}{0}
%\setcounter{table}{0}
\setcounter{secnumdepth}{4}
\setcounter{subsection}{0} 
\setcounter{subsubsection}{0}
\usecounter{subsubsection}

==> commondefs2.tex <==
\newcommand{\vbdlspacing}{\\[-15pt]}
\newcommand{\vbabovecaption}{\vspace{-24pt}}
\newcommand{\vbbelowcaption}{\vspace{-12pt}}
\newcommand{\vbabove}{\vspace{-12pt}}
\newcommand{\vbbelow}{\vspace{-12pt}}
\newcommand{\itemspace}{\vspace{-6pt}}

\begin{comment}
\renewcommand{\thepage}{\arabic{chapter}.\arabic{section}-\arabic{page}}
\renewcommand{\thefigure}{\arabic{chapter}.\arabic{section}-\arabic{figure}}
\renewcommand{\thetable}{\arabic{chapter}.\arabic{section}-\arabic{table}}
\end{comment}
\renewcommand\floatpagefraction{.95}
\renewcommand\topfraction{.95}
\renewcommand\bottomfraction{.95}
\renewcommand\textfraction{.05}   


==> costs/resetcounters.tex <==
%\setcounter{page}{1}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{secnumdepth}{4}
\setcounter{subsection}{0} 
\setcounter{subsubsection}{0}
\usecounter{subsubsection}

==> resetcounters2.tex <==
%\setcounter{page}{1}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{secnumdepth}{4}
\setcounter{subsection}{0} 
\setcounter{subsubsection}{0}
\usecounter{subsubsection}

==> resetcounters_VB.tex <==
%\setcounter{page}{1}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{secnumdepth}{4}
\setcounter{subsection}{0} 
\setcounter{subsubsection}{0}
\usecounter{subsubsection}

==> sites/resetcounters.tex <==
%\setcounter{page}{1}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{secnumdepth}{4}
\setcounter{subsection}{0} 
\setcounter{subsubsection}{0}
\usecounter{subsubsection}

==> trc_style.tex <==
%
% This file contains modified section and bibliography 
% headings. It is modified from the standard book class 
% file of LaTeX2e for the ILC-TRC report.
% R. Reitmeyer
% SLAC TechPubs
% 31 October 2002
%
%

% Makes Chapter titles flushright
\def\@makechapterhead#1{%
  \vspace*{50\p@}%
  {\parindent \z@ \flushright \normalfont
    \ifnum \c@secnumdepth >\m@ne
      \if@mainmatter
        \huge\bfseries \@chapapp\space \thechapter
        \par\nobreak
        \vskip 20\p@
      \fi
    \fi
    \interlinepenalty\@M
    \Huge \bfseries #1\par\nobreak
    \vskip 40\p@
  }}

% Makes TOC, LOF, and LOT titles flushright
\def\@makeschapterhead#1{%
  \vspace*{50\p@}%
  {\parindent \z@ \flushright
    \normalfont
    \interlinepenalty\@M
    \Huge \bfseries  #1\par\nobreak
    \vskip 40\p@
  }}

% Resets some programmed text to be in all caps.
\renewcommand{\bibname}{\sffamily BIBLIOGRAPHY for CHAPTER \thechapter}

\renewcommand\figurename{\sffamily\small FIGURE}
\renewcommand\tablename{\sffamily\small TABLE}

\renewcommand\contentsname{\sffamily CONTENTS}
\renewcommand\listfigurename{\sffamily LIST of FIGURES}
\renewcommand\listtablename{\sffamily LIST of TABLES}
\renewcommand\chaptername{\sffamily CHAPTER}

% Resets the sectioning commands (for formatting and style).
\renewcommand\section{\@startsection {section}{1}{\z@}%
                                   {-4ex \@plus -1ex \@minus -.2ex}%
                                   {2.5ex \@plus.2ex}%
                                   {\sffamily\Large\bfseries\MakeUppercase}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
                                     {-3.25ex\@plus -1ex \@minus -.2ex}%
                                     {1.25ex \@plus .2ex}%
                                     {\sffamily\Large\bfseries}}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                                     {-3.25ex\@plus -1ex \@minus -.2ex}%
                                     {1.25ex \@plus .2ex}%
                                     {\sffamily\large\bfseries}}
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
                                    {3.25ex plus 1ex minus .2ex}%
                                    {-2em}%
                                    {\sffamily\normalsize\bfseries}}
\renewcommand\subparagraph{\@startsection{subparagraph}{5}{\z@}%
                                       {3.25ex plus 1ex minus .2ex}%
                                       {-2em}%
                                      {\sffamily\normalsize\bfseries}}

% Prints out Equation with equation numbers.
\renewcommand\theequation
  {\textsf{\@roman\c@equation}}





%% Messing with the text around a caption for figures and tables
%\def\fnum@figure{\figurename~\thefigure}
%\def\fnum@table{\tablename~\thetable}
%
%\setlength\abovecaptionskip{10\p@}
%\setlength\belowcaptionskip{10\p@}
%\long\def\@makecaption#1#2{%
%  \vskip\abovecaptionskip
%  \sbox\@tempboxa{#1   \\#2\par}%
%  \ifdim \wd\@tempboxa >\hsize
%   #1   \\#2\par
% \else
%    \global \@minipagefalse
%    \hb@xt@\hsize{\hfil\box\@tempboxa\hfil}%
%  \fi
%  \vskip\belowcaptionskip}

%
% Stolen from Elsevier Science Publishers style file espcrc2.sty.
% Annoyingly, this does NOT correct table captions for rotated tables. That's OK, since space is usually
% at a premium there.
%
\long\def\@makefigurecaption#1#2{\vskip 10mm #1. #2\par}

\long\def\@maketablecaption#1#2{\hbox to \hsize{\parbox[t]{\hsize}
  {#1 \\ #2}}\vskip 1ex}

\def\fnum@figure{\sffamily\small FIGURE \thefigure}
\def\figure{\let\@makecaption\@makefigurecaption \@float{figure}}
\@namedef{figure*}{\let\@makecaption\@makefigurecaption \@dblfloat{figure}}

% \def\fnum@table{\sffamily\small TABLE \thetable}
\def\table{\let\@makecaption\@maketablecaption \@float{table}}
\@namedef{table*}{\let\@makecaption\@maketablecaption \@dblfloat{table}}

\floatsep 8mm plus 4pt minus 4pt % Space between adjacent floats moved
                                  % to top or bottom of text page.
\textfloatsep=\floatsep           % Space between main text and floats
                                  % at top or bottom of page.
\intextsep=\floatsep              % Space between in-text figures and 
                                  % text.


